ColdNAS: Search to Modulate for User Cold-Start Recommendation

Making personalized recommendation for cold-start users, who only have a few interaction histories, is a challenging problem in recommendation systems. Recent works leverage hypernetworks to directly map user interaction histories to user-specific parameters, which are then used to modulate predictor by feature-wise linear modulation function. These works obtain the state-of-the-art performance. However, the physical meaning of scaling and shifting in recommendation data is unclear. Instead of using a fixed modulation function and deciding modulation position by expertise, we propose a modulation framework called ColdNAS for user cold-start problem, where we look for proper modulation structure, including function and position, via neural architecture search. We design a search space which covers broad models and theoretically prove that this search space can be transformed to a much smaller space, enabling an efficient and robust one-shot search algorithm. Extensive experimental results on benchmark datasets show that ColdNAS consistently performs the best. We observe that different modulation functions lead to the best performance on different datasets, which validates the necessity of designing a searching-based method.

==> coldnas-alt-text.tex <==
Figure 1: \Description{Figure 1 is an illustration of user cold-start models.}

Figure 2: \Description[Figure 2 shows the original and transformed search space, and the structure of supernet.]{Figure 2(a) shows the original search space in the form of binary tree. For the leaf nodes, the deepest one represents the output of hidden layer in predictor $\mathbf{h}^l$, each of the others represents a group of user-specific parameter $\mathbf{phi}_i^c$. For the intermediate nodes, a binary operation is specified, representing the output of this operation taking its two child nodes. There are $C+1$ leaf nodes. Going through the deepest leaf to the root is the procedure of a modulation.
Figure 2(b) shows the transformed search space in the form of binary tree. The meaning of leaf nodes is the same as figure 2(a) and the structure is similar. But there is only 5 leaf nodes. The operation on the 4 non-leaf nodes exactly forms the operation set containing max, min, multiply and add in any order.
Figure 2(c) shows the structure of one layer l in the supernet. the input is $\mathbf{h}^l$, which is modulated by 4 steps sequentially. The output of each step $k$ is the sum of weight $\alpha^l,k+1$ times the operated and 1 minus the weight times the un-operated. The operations of the 4 steps are max, min, multiply and add in any order.}

Figure 3: \Description[ColdNAS finds the best model taking the shortest time comparing with other search strategies.]{The curve of testing MSE vs clock time on MovieLens, BookCrossing and Last.fm. There are curves of 4 search strategies: ColdNAS, ColdNAS-Bilevel, Random (C=4) and Random (T). On any dataset, ColdNAS finds the best model taking the shortest time. ColdNAS-Bilevel is the second fastest. Random (T) is the third fastest. Random (C=4) is the slowest.}

Figure 4: \Description[ColdNAS finds the best model taking the shortest time comparing with other search spaces.]{The curve of testing MSE vs clock time on MovieLens, BookCrossing and Last.fm. There are 6 curves: ColdNAS, Random (C from 1 to 4) and Random (T). On any dataset, ColdNAS finds the best model taking the shortest time. Random (T) is the second fastest and finds the same best model. Random (C from 1 to 4) searches slower with the growth of C value, while the finally found model performs better but all perform worse than the previous two. }

Figure 5: \Description[Sensitivity analysis of $K$, depth of predictor, support set size on Last.fm.]{Figure 5 shows Model sensitivity analysis on Last.fm.
Figure 5(a) shows the MSE and $\text{nDCG}_5$ of different $K$. With $K$ growing from 0 to 16, MSE first drops than grows, $\text{nDCG}_5$ first grows than drops.
Figure 5(b) shows the MSE and $\text{nDCG}_5$ of different depth of predictor. When the layer number grows from 2 to 5, MSE first drops then grows and reaches the lowest point at 3 layers, $\text{nDCG}_5$ first grows then stay almost still from 3 to 5. 
Figure 5(c) shows the MSE and $\text{nDCG}_5$ of different support set size. When the sample number in support set grows from 5 to 20, MSE drops and $\text{nDCG}_5$ grows. With any support set size, the MSE of ColdNAS is always lower than TaNP and the $\text{nDCG}_5$ is always higher.}

Figure 6: \Description[Heat maps of $\mathbf{\alpha}$ and performance curve to support an adaptation network with 2 layers is expressive enough.]{Figure 6 shows evidence of an adaptation network with 2 layers is expressive enough. Figure 6(a)~(c) visualize the 4*4 $\alpha^{l,k}$s values with different depth of adaptation network, from 2 layers to 5 layers. The visualizations look almost identical. Figure 6(e) shows the curve of depth of adaptation network vs testing MSE, which is almost horizontal.}

Figure 7: \Description[Heat maps of $\mathbf{\alpha}$ to verify the properties in transformed space. ]{Figure 7 verifies the the inner-group consistence and permutation-invariance by visualizing the $\{\alpha^{l,k}\}$. Figure 7(a) visualizes the $\{\alpha^{l,k}\}$ after changing add to sub, which is almost identical with the unchanged.  Figure 7(b) visualizes the $\{\alpha^{l,k}\}$ after changing multiply to divide , which is also almost identical with the unchanged.  Figure 7(c) visualizes the $\{\alpha^{l,k}\}$ after permuting the 4 operations in the supernet, where $\alpha^{l,k}$s  look permuted along with the operations.}

Figure 8: \Description[Sensitivity analysis of $K$, depth of predictor, support set size on MovieLens. ]{Figure 8 shows model sensitivity analysis on MovieLens.
Figure 8(a) shows the MSE and $\text{nDCG}_5$ of different $K$. With $K$ growing from 0 to 16, the curves fluctuate while MSE first shows a dropping trend than shows a growing trend, $\text{nDCG}_5$ first shows a growing trend than shows a dropping trend.
Figure 8(b) shows the MSE and $\text{nDCG}_5$ of different depth of predictor. When the layer number grows from 2 to 5, MSE keeps dropping, $\text{nDCG}_5$ first grows then stays almost still from 4 to 5.
Figure 8(c) shows the MSE and $\text{nDCG}_5$ of different support set size. When the sample number in support set grows from 5 to 20, MSE drops and $\text{nDCG}_5$ grows.}

Figure 9: \Description[Sensitivity analysis of $K$, depth of predictor, support set size on BookCrossing.]{Figure 9 shows model sensitivity analysis on BookCrossing.
Figure 9(a) shows the MSE and $\text{nDCG}_5$ of different $K$. With $K$ growing from 0 to 16, the curves fluctuates while MSE first shows a dropping trend than shows a growing trend, $\text{nDCG}_5$ first shows a growing trend than shows a dropping trend.
Figure 9(b) shows the MSE and $\text{nDCG}_5$ of different depth of predictor. When the layer number grows from 2 to 5, MSE keeps dropping, $\text{nDCG}_5$ first grows then stay almost still from 3 to 5.
Figure 9(c) shows the MSE and $\text{nDCG}_5$ of different support set size. When the sample number in support set grows from 5 to 20, MSE drops and $\text{nDCG}_5$ grows.}
